Scale Effects in Ridesplitting: A Case Study of the City of Chicago

Ridesplitting -- a type of ride-hailing in which riders share vehicles with other riders -- has become a common travel mode in some major cities. This type of shared ride option is currently provided by transportation network companies (TNCs) such as Uber, Lyft, and Via and has attracted increasing numbers of users, particularly before the COVID-19 pandemic. Previous findings have suggested ridesplitting can lower travel costs and even lessen congestion by reducing the number of vehicles needed to move people. Recent studies have also posited that ridesplitting should experience positive feedback mechanisms in which the quality of the service would improve with the number of users. Specifically, these systems should benefit from economies of scale and increasing returns to scale. This paper demonstrates evidence of their existence using trip data reported by TNCs to the City of Chicago between January and September 2019. Specifically, it shows that increases in the number of riders requesting or authorizing shared trips during a given time period is associated with shorter trip detours, higher rates of riders being matched together, lower costs relative to non-shared trips, and higher willingness for riders to share trips.

==> Scale Effects in Ridesplitting Updated/labels-cost_ratio_revised2.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Sat, Dec 03, 2022 - 9:39:25 PM
\begin{table}[!htbp] \centering 
  \caption{Regression results for cost ratio} 
  \label{tab:cost_ratio_revised} 
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
\\[-1.8ex] & Time-based $e^t$ & Distance-based $e^d$ \\ 
\hline \\[-1.8ex] 
 $\sqrt{n^a(h,d,m)}$ & $-$0.0002$^{***}$ & $-$0.001$^{***}$ \\ 
  & (0.00004) & (0.00004) \\ 
  AM Peak & $-$0.066$^{***}$ & $-$0.026$^{***}$ \\ 
  & (0.004) & (0.003) \\ 
  Mid-day & $-$0.014$^{***}$ & 0.012$^{***}$ \\ 
  & (0.003) & (0.003) \\ 
  PM Peak & $-$0.022$^{***}$ & 0.001 \\ 
  & (0.004) & (0.003) \\ 
  Constant & 0.524$^{***}$ & 0.654$^{***}$ \\ 
  & (0.003) & (0.003) \\ 
 \hline \\[-1.8ex] 
R$^{2}$ & 0.256 & 0.571 \\ 
Adjusted R$^{2}$ & 0.254 & 0.570 \\ 
\hline 
\hline \\[-1.8ex] 
Significance levels & \multicolumn{2}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Scale Effects in Ridesplitting Updated/labels-detour_disaggregate_Jan_Sep.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Feb 14, 2023 - 2:37:05 PM
\begin{table}[!htbp] \centering 
  \caption{Regression results for detour distance (mile)} 
  \label{tab:detour_disaggregate} 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{6}{c}{Detour distance $de^{O,D}(h,d,m)$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 $\frac{1}{n^{O,D}_{s_m}(h,d,m)}$ & 0.341$^{***}$ & 0.234$^{***}$ & 0.380$^{***}$ & 0.424$^{***}$ & 0.431$^{***}$ & 0.330$^{***}$ \\ 
  & (0.060) & (0.047) & (0.058) & (0.057) & (0.122) & (0.056) \\ 
  Constant & 0.348$^{***}$ & 0.238$^{***}$ & 0.231$^{***}$ & 0.266$^{***}$ & 0.145$^{*}$ & 0.219$^{***}$ \\ 
  & (0.036) & (0.031) & (0.040) & (0.037) & (0.083) & (0.036) \\ 
 \hline \\[-1.8ex] 
R$^{2}$ & 0.033 & 0.029 & 0.048 & 0.059 & 0.014 & 0.040 \\ 
Adjusted R$^{2}$ & 0.032 & 0.028 & 0.047 & 0.058 & 0.013 & 0.039 \\ 
\hline 
\hline \\[-1.8ex] 
Significance levels & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Scale Effects in Ridesplitting Updated/labels-detour_disaggregate_Jan_Sep_7-16.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Wed, Feb 15, 2023 - 12:14:30 PM
\begin{table}[!htbp] \centering 
  \caption{Regression results for detour distance (mile)} 
  \label{tab:detour_disaggregate_7_16} 
\begin{tabular}{@{\extracolsep{5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{Detour distance $de^{O,D}(h,d,m)$} \\ 
\\[-1.8ex] & (7) & (8) & (9) & (10) & (11)\\ 
\hline \\[-1.8ex] 
 $\frac{1}{n^{O,D}_{s_m}(h,d,m)}$ & 0.312$^{***}$ & 0.985$^{***}$ & 0.351$^{***}$ & 0.355$^{***}$ & 0.415 \\ 
  & (0.050) & (0.230) & (0.061) & (0.052) & (0.272) \\ 
  Constant & 0.293$^{***}$ & 0.927$^{***}$ & 0.166$^{***}$ & 0.240$^{***}$ & 0.324$^{*}$ \\ 
  & (0.032) & (0.181) & (0.044) & (0.035) & (0.195) \\ 
 \hline \\[-1.8ex] 
R$^{2}$ & 0.039 & 0.021 & 0.035 & 0.047 & 0.005 \\ 
Adjusted R$^{2}$ & 0.038 & 0.020 & 0.034 & 0.046 & 0.003 \\ 
\hline 
\hline 
\\[-1.8ex] & (12) & (13) & (14) & (15) & (16)\\ 
\hline \\[-1.8ex] 
 $\frac{1}{n^{O,D}_{s_m}(h,d,m)}$ & 0.519$^{***}$ & 1.434$^{***}$ & 1.298$^{***}$ & 0.820$^{***}$ & 0.266$^{***}$ \\ 
  & (0.061) & (0.194) & (0.257) & (0.190) & (0.043) \\ 
  Constant & 0.217$^{***}$ & 0.790$^{***}$ & 0.988$^{***}$ & 0.979$^{***}$ & 0.228$^{***}$ \\ 
  & (0.034) & (0.130) & (0.188) & (0.144) & (0.031) \\ 
 \hline \\[-1.8ex] 
R$^{2}$ & 0.088 & 0.052 & 0.029 & 0.021 & 0.045 \\ 
Adjusted R$^{2}$ & 0.087 & 0.051 & 0.028 & 0.020 & 0.044 \\ 
\hline 
\hline \\[-1.8ex] 
Significance levels & \multicolumn{5}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Scale Effects in Ridesplitting Updated/labels-matching_rate_revised2.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Sat, Dec 03, 2022 - 7:42:47 PM
\begin{table}[!htbp] \centering 
  \caption{Regression results for matched percentage of shared trips} 
  \label{tab:matching_rate_revised} 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & \multicolumn{3}{c}{Matched percentage $\theta_{s_m,i}(h,d,m)$} \\ 
\\[-1.8ex] & N Jan-Sep & S Jan-Sep before & S Jan-Sep after\\ 
\hline \\[-1.8ex] 
 $\sqrt{n_{s_a,i}^a(h,d,m)}$ & 0.546$^{***}$ & 0.859$^{***}$ & 1.378$^{***}$ \\ 
  & (0.013) & (0.071) & (0.051) \\ 
  AM Peak & $-$0.120 & $-$5.704$^{***}$ & $-$4.255$^{***}$ \\ 
  & (0.455) & (0.996) & (0.646) \\ 
  Mid-day & $-$4.535$^{***}$ & $-$8.234$^{***}$ & $-$6.745$^{***}$ \\ 
  & (0.362) & (0.843) & (0.549) \\ 
  PM Peak & $-$5.083$^{***}$ & $-$8.621$^{***}$ & $-$7.831$^{***}$ \\ 
  & (0.429) & (0.904) & (0.584) \\ 
  Constant & 55.515$^{***}$ & 58.172$^{***}$ & 50.326$^{***}$ \\ 
  & (0.335) & (0.573) & (0.512) \\ 
 \hline \\[-1.8ex] 
R$^{2}$ & 0.631 & 0.096 & 0.372 \\ 
Adjusted R$^{2}$ & 0.631 & 0.094 & 0.370 \\ 
\hline 
\hline \\[-1.8ex] 
Significance levels & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

